Stroke3D: Lifting 2D strokes into rigged 3D model via latent diffusion models

Rigged 3D assets are fundamental to 3D deformation and animation. However, existing 3D generation methods face challenges in generating animatable geometry, while rigging techniques lack fine-grained structural control over skeleton creation. To address these limitations, we introduce Stroke3D, a novel framework that directly generates rigged meshes from user inputs: 2D drawn strokes and a descriptive text prompt. Our approach pioneers a two-stage pipeline that separates the generation into: 1) Controllable Skeleton Generation, we employ the Skeletal Graph VAE (Sk-VAE) to encode the skeleton's graph structure into a latent space, where the Skeletal Graph DiT (Sk-DiT) generates a skeletal embedding. The generation process is conditioned on both the text for semantics and the 2D strokes for explicit structural control, with the VAE's decoder reconstructing the final high-quality 3D skeleton; and 2) Enhanced Mesh Synthesis via TextuRig and SKA-DPO, where we then synthesize a textured mesh conditioned on the generated skeleton. For this stage, we first enhance an existing skeleton-to-mesh model by augmenting its training data with TextuRig: a dataset of textured and rigged meshes with captions, curated from Objaverse-XL. Additionally, we employ a preference optimization strategy, SKA-DPO, guided by a skeleton-mesh alignment score, to further improve geometric fidelity. Together, our framework enables a more intuitive workflow for creating ready to animate 3D content. To the best of our knowledge, our work is the first to generate rigged 3D meshes conditioned on user-drawn 2D strokes. Extensive experiments demonstrate that Stroke3D produces plausible skeletons and high-quality meshes.

==> Sup_figtex/mesh_compare.tex <==
\begin{figure}[ht!]   % [t] 表示图片放置在页面顶部
    \centering
    \includegraphics[width=\textwidth]{Sup_figs/mesh_compare.pdf} % 图片路径及宽度设置
    % \vspace{-2 em}
    \caption{\textbf{More generated mesh comparison.}}
    \label{sup:mesh_compare2} % 标签用于引用
    % \vspace{-1 em}
\end{figure}

==> fig_tex/ablation_struct.tex <==
\setlength{\intextsep}{0pt} % 这会移除图和周围文本之间的垂直间距
\begin{wrapfigure}{r}{0.4\textwidth} % 调整这里，将整个wrapfigure的宽度设置为0.35倍的文本宽度
    \centering
    \includegraphics[width=0.4\textwidth, height=4cm]{figs/ablation_struct_v2.pdf} % 调整这里，将图片宽度设置为0.35倍的文本宽度
    % \vspace{-2em} % 负间距，可以尝试保留或删除，看效果。图片变小后，可能不需要那么多负间距了
    \caption{\textbf{Ablation study on structural condition.} With structral condition, the model converge faster. The pink and blue regions indicate the intervals where the loss decreases rapidly.}
    \vspace{-0.5 em} 
    % 如果 caption 和下面的文本距离太远，可以稍微负一些
    \label{fig:ablation_study}
\end{wrapfigure}

==> sec/3_preliminary.tex <==
\section{Preliminaries}
% \input{fig_tex/caption}
\textbf{Diffusion Models.} Diffusion probabilistic models \citep{ho2020denoising, song2020score} aim to learn the underlying data distribution \( p_{\mathrm{data}} \) through a progressive denoising process. The model is described as a discrete-time stochastic process \( \{ \bm{x}_t \}_{t=0}^T \), where \( \bm{x}_0 \sim p_{\mathrm{data}} \), and for each timestep, \( \bm{x}_t \sim \mathcal{N}(\bm{x}_{t-1}; \sqrt{\alpha_t / \alpha_{t-1}} \bm{x}_{t-1}, (1 - \alpha_t / \alpha_{t-1}) \bm{I}) \). Here the scalar \( \alpha_t \) progressively controls the noise, with the boundary conditions \( \alpha_0 = 1 \) and \( \alpha_T \approx 0 \). This process for adding noise as follows:
\begin{equation}
    \bm{x}_t = \sqrt{\alpha_t} \bm{x}_0 + \sqrt{1 - \alpha_t} \bm{\epsilon}, \quad \text{where} \quad \bm{\epsilon} \sim \mathcal{N}(\bm{0}, \bm{I}).
\end{equation}
A diffusion model \( \epsilon_{\phi} \) is trained to estimate the noise \( \epsilon \) from \( \bm{x}_t \), with the training loss formulated as:
\begin{equation}
    \mathcal{L} = \mathbb{E}_{\bm{x}_0, t, \bm{\epsilon}} \left[ \left\| \epsilon_{\bm{\phi}} \left( \sqrt{\alpha_t}\bm{x}_0 + \sqrt{1 - \alpha_t}\bm{\epsilon}, t, \bm{C} \right) - \bm{\epsilon} \right\|_2^2 \right],
\end{equation}
where \( \bm{C} \) represents any conditioning signals, such as text or images.



\textbf{Graph Neural Networks.} The message-passing paradigm is the foundational principle for a majority of Graph Neural Networks (GNNs), including seminal models like GCN \citep{kipf2016semi} , GAT \citep{velivckovic2017graph} and TransformerConv \citep{shi2020masked}. These models computes node embeddings by repeatedly aggregating information from adjacent nodes and refining them with a non-linear function. The propagation step can be written as:
\begin{equation}
    z_i^{(l)} = U \left( h_i^{(l-1)}, M \left( \left\{ z_j^{(l-1)}, z_i^{(l-1)} \right\} \mid v_j \in N_i \right) \right)
\end{equation}

Here, \( z_i^{(l)} \) is the feature of node \( i \) at layer \( l \) and \( N_i \) denotes its set of neighboring nodes \(v \). The function \( M \) aggregates features from the nodes in \( N_i \), while the update function \(U\) combines this aggregated message with the central node's feature to produce its new embedding.

==> table_tex/fid_eval.tex <==
\begin{table*}[ht]
\centering
\caption{\textbf{Quantitative comparison of FID score.} FID scores are calculated over five categories. The lowest
scores among all methods are bold and the lowest scores among baseline methods are underlined.}
\vspace{0.4em}
\footnotesize
\begin{tabular}{l|ccccc}
\hline
\textbf{Method\textbackslash{}FID Score $\downarrow$} & \textbf{All} & \textbf{Anthro.} & \textbf{Character} & \textbf{Animal} & \textbf{Plant} \\
\hline
\rowcolor[HTML]{F9FFF9}RigNet & 2.539 & 4.644 & 0.784 & 0.873 & 5.260 \\
\rowcolor[HTML]{F9FFF9}SKDream & 1.387 & 1.727 & 3.206 & 0.674 & 4.030 \\
\rowcolor[HTML]{F9FFF9}MagicArticulation & \textbf{0.092} & \textbf{0.239} & \textbf{0.137} & \textbf{0.084} & \textbf{0.471} \\
\hline
\rowcolor[HTML]{F9FBFF}\textbf{Ours (GnnDiff)} & \underline{1.184} & \underline{1.203} & \underline{0.570} & \underline{1.972} & \underline{2.343} \\
\hline
\end{tabular}
\vspace{-1em}
\label{table:fid_eval}
\end{table*}

